Detecting Grasping Sites in a Martian Lava Tube: Multi-Stage Perception Trade Study for ReachBot

This paper presents a trade study analysis to design and evaluate the perception system architecture for ReachBot. ReachBot is a novel robotic concept that uses grippers at the end of deployable booms for navigation of rough terrain such as walls of caves and lava tubes. Previous studies on ReachBot have discussed the overall robot design, placement and number of deployable booms, and gripper mechanism design; however, analysis of the perception and sensing system remains underdeveloped. Because ReachBot can extend and interact with terrain over long distances on the order of several meters, a robust perception and sensing strategy is crucial to identify grasping locations and enable fully autonomous operation. This trade study focuses on developing the perception trade space and realizing such perception capabilities for a physical prototype. This work includes analysis of: (1) multiple-range sensing strategies for ReachBot, (2) sensor technologies for subsurface climbing robotics, (3) criteria for sensor evaluation, (4) positions and modalities of sensors on ReachBot, and (5) map representations of grasping locations. From our analysis, we identify the overall perception strategy and hardware configuration for a fully-instrumented case study mission to a Martian lava tube, and identify specific sensors for a hardware prototype. The final result of our trade study is a system design conducive to benchtop testing and prototype hardware development.

==> 1_Introduction.tex <==
Skylights and caves on Mars and the Moon could yield  astrobiological samples, unlock answers for geological origins, and reveal a previously undiscovered subsurface world. While there is clear scientific value in such environments, exploring them is a daunting technical challenge: navigating perilous, unknown terrain requires an innovative solution capable of versatile mobility through loose material and unpredictable obstacles. ReachBot is a robot concept that answers this call for mobility in extreme environments.

\begin{figure}
\includegraphics[width=3.25in]{figures/reachbotconcept.png}
\caption{A diagram illustrating different ReachBot configuration concepts for a martian lava tube mission. (A) shows a ReachBot configuration concept using extendable booms. An eight-boom configuration has been explored in previous work. At the end of each boom is a microspine gripper that can grasp onto rough surfaces. (B) is an image of a ReachBot microspine gripper previously tested on lava tube rocks. (C) shows a ReachBot configuration that combines cables with booms for placing the grippers.}
\label{fig:reachbotconcepts}
\end{figure}

As discussed in previous work \cite{schneider2022reachbot,chen2022reachbot,newdick2023designing,newdick2023motion,roberts2023skeleton}, ReachBot's limbs are extendable booms that act as prismatic joints to achieve a large workspace compared to traditional rigid-link designs. These steerable booms, when paired with grippers, enable ReachBot to climb and span steep verticals inside caverns that a jumping robot or aerial robot may fail to access, as shown in Fig.~\ref{fig:reachbotconcepts}(A,B). Furthermore, the booms could also be combined with other technologies, such as cables or tethers as shown in Fig.~\ref{fig:reachbotconcepts}(C), to further increase reach and reduce mass and volume complexity. ReachBot's large workspace expands the number of reachable anchor points in the environment, which is especially advantageous in unknown environments with sparse anchor points or obstructions in terrain.

To grasp the environment, the gripper at the end of each boom is equipped with microspines. Microspines have been used in multiple works to grasp rough and rocky surfaces, including for planetary exploration \cite{asbeck2006scaling,parness2017lemur,wang2019spinyhand,backus2020design,pope2016multimodal}, and several works have analyzed the conditions for successful grasping with microspines \cite{jiang2018stochastic,wang2019spinyhand,asbeck2012designing}. As shown in Fig.~\ref{fig:reachbotconcepts}(B), the ReachBot gripper successfully grasps surface locations that are approximately convex.

While ReachBot's mechanical architecture and motion planning have been extensively studied, analysis of the perception system trade space has been comparatively scant. Early work indoors assumed known grasping locations as captured by overhead cameras \cite{chen2022reachbot}. Later, a two-stage perception strategy and sensor system was introduced in a successful field testing demonstration in a Mojave Desert lava tube \cite{chen2024locomotion}, but this only used RGB-D images in daylight and did not review other sensing modalities or mission-level considerations. Although RGB-D images work in the field, alternatives should be investigated for more realistic mission conditions. To operate in caves and skylights, every perception system faces the typical subsurface concerns---low power, limited communication bandwidth, total darkness, and dusty conditions. These are in addition to and compounded by the operational challenges of any space hardware---radiation hardening, thermal requirements, mass/volume restrictions, cost, and technological risk. Because ReachBot has a much larger workspace than that of a typical climbing robot, examination of high-level sensing strategies is also warranted. 

\subsubsection{Statement of Contributions}

This work evaluates perception system approaches that enable ReachBot to identify grasping sites, building upon previous ReachBot analysis as well as existing work for subsurface robots that use distance-based sensing. The main contributions of this work are:
\begin{itemize}
    \item We present a survey of different robotic sensing modalities for a climbing robot in a subsurface environment.
    \item  We discuss perception system strategies and candidate map outputs of a ReachBot perception system
    \item We propose evaluation criteria of sensor hardware for a configuration of ReachBot that discerns grasping locations in a martian lava tube environment.
    \item We conduct trades and propose a hardware configuration that could be physically prototyped for testing in a lava tube environment.
\end{itemize}

\subsubsection{Paper Organization} The rest of this paper is organized as follows. Section \ref{sec:background} describes background literature on the perception systems of robots designed for either climbing with microspines or subsurface exploration. We also discuss considerations for upstream trades around choice of perception strategy, and downstream trades on choice of environment representation for the planner. Section \ref{sec:tradestudy} discusses the trade study process. Then we develop evaluation criteria for sensor selection in Section \ref{sec:componentanalysis} and present the viable perception architectures in Section \ref{sec:sensorresults} for a specific ReachBot mission. We follow with analysis of the different map representation choices in Section \ref{sec:graspingrepresentations}. Finally, we provide conclusions and suggest next steps for this work.

\begin{figure*}
\centering
\includegraphics[width=6in]{figures/tradestudyflowchart}
\caption{A flowchart depicting the trade study process in this work detailed in Section \ref{sec:tradestudy}, which begins with the dictation of Science Goals for the mission. Initial engineering trades (dark green) are derived from science parameters, with perception requirements (light green) further derived downstream.}
\label{fig:tradestudyflowchart}
\end{figure*}

==> 2_Background.tex <==
\subsection{Perception Considerations for Microspine Robots}

Others have built robotic systems using microspines for climbing. Most notably, LEMUR 3 from JPL is a multi-limbed robot that was field tested in a lava tube environment; their perception system was an actuated LiDAR system on the body to construct a map of grasping locations \cite{parness2017lemur,uckert2020investigating}. We note however that LEMUR and its variants are all climbing robots that hug the rock wall, enabling body-mounted sensors to return highly dense and informative geometric reconstructions. ReachBot meanwhile climbs by pulling on the environment with potentially extra-long limbs. A body-mounted sensor on ReachBot will almost always return much sparser data compared to a more traditional climbing robot due to the increased distance from the rock walls. Therefore, designing the perception system for ReachBot requires more attention to criteria involving scene reconstruction from afar.

\subsection{Perception for Exploration in Subterranean Environments}

Perception systems for autonomous navigation in confined and subterranean spaces have been carefully evaluated, most recently with the DARPA Subterranean Challenge, which involved teams of robots searching for and detecting artifacts placed in an unknown subterranean environment \cite{chung2023into}. There are a number of relevant surveys and challenge retrospectives \cite{tranzatto2022cerberus,agha2021nebula,ebadi2022present,hudson2021heterogeneous,azpurua2023survey} that discuss in further detail the learnings from this Challenge.

Of import is that the majority of teams used a combination of LiDAR and IMU as the primary sensing component. LiDAR units return accurate long-range depth measurements and are illumination invariant; IMUs are not sensitive to environmental disturbances and help distinguish between places with the same perceptual appearance \cite{tranzatto2022cerberus}. Various other types of sensing (e.g. vision, thermal, odometry) is used in addition to LiDAR to increase redundancy especially when there are adverse conditions \cite{ebadi2022present}. Multimodal perception, especially that combining LiDAR with another modality, continues to be investigated for subsurface robotics \cite{miki2022learning,dharmadhikari2021autonomous}. Many teams also designed the perception system payload to be modular, allowing for standardized calibration and decoupling the system from other hardware. 

\subsection{ReachBot Perception Strategy Considerations}
 
The perception system must generate a map of grasping sites for the planner. Because booms lose pointing accuracy when extended long distances, making the correction of large positional errors cumbersome, a two-stage strategy has been proposed \cite{chen2024locomotion}. This involves a single RGB-D camera mounted on a boom, which first perceived regions of interest from afar (boom in a stowed position), and then finalized the grasping site locations when the boom deploys closer to the surface. Here, we discuss the perception strategies for ReachBot more generally. 

A one-stage perception process involves a perception sensor suite only mounted on the main body of ReachBot. We assume the use of multiple sensors in this sensor suite because the body of ReachBot can hold more mass than the booms, and multiple sensors reduce the risk that ReachBot cannot perceive its surroundings. However, for ReachBots with multiple long-range booms that can extend dozens of meters in large-diameter lava tubes, the aforementioned pointing accuracy becomes an issue. It follows that a one-stage perception process is better suited for a ReachBot configuration with short booms for a narrow space such as a slim vent. In other words, one-stage perception process allows for only far-field sensing, and perceived spatial resolution (thus accuracy) does not scale with boom length.

A two-stage perception process of both far-field and near-field sensing has the benefit of additional sampling, which increases accuracy in grasping site predictions. This process does pose an additional requirement: either having a lightweight sensor mounted on the distal end of the boom to enable near-range sampling (in addition to or in place of a body sensor), or a motion planning procedure to bring a body-mounted sensor closer to the desired surface. Implementation of the former for multiple booms depends on the permissible mass budget of the boom and the scale of distances covered. The latter could be accomplished with more stringent stance planning, or with hybrid locomotion schemas such as rolling and climbing. 

A related question is whether there should be any gripper-level sensing, for perceiving contact. One may then implement all three scales of sensing: far-field, near-field, and gripper-based sensing (or a subset). Instrumenting microspine grippers with force-torque, proximity, or tactile sensing could yield a number of benefits. A benefit is that estimating distance of the gripper to the surface could be used in a feedback loop to trigger the grasping sequence onto a surface (in previous tests, grasping sequences were always triggered manually). Force-torque information at the wrist could also be used for detecting gripper contact and monitoring grasping events. Sensor choice on the distal end must trade against the permissible mass budget of the boom.
